A pseudo-likelihood approach to community detection in weighted networks

Community structure is common in many real networks, with nodes clustered in groups sharing the same connections patterns. While many community detection methods have been developed for networks with binary edges, few of them are applicable to networks with weighted edges, which are common in practice. We propose a pseudo-likelihood community estimation algorithm derived under the weighted stochastic block model for networks with normally distributed edge weights, extending the pseudo-likelihood algorithm for binary networks, which offers some of the best combinations of accuracy and computational efficiency. We prove that the estimates obtained by the proposed method are consistent under the assumption of homogeneous networks, a weighted analogue of the planted partition model, and show that they work well in practice for both homogeneous and heterogeneous networks. We illustrate the method on simulated networks and on a fMRI dataset, where edge weights represent connectivity between brain regions and are expected to be close to normal in distribution by construction.

==> acknowledgments.tex <==
\section{Acknowledgments}

The authors thank Min Xu, Varun Jog and Po-Ling Loh for sharing their code with us. The authors also would like to thank Keith Levin for sharing the networks average from the COBRE data set.

AC was supported by grant \#2018/18115-2 S\~ao Paulo Research Foundation (FAPESP). This work was developed
while AC was a Visiting Postdoctoral Researcher at University of Michigan. She thanks the support and
hospitality of this institution.

==> pseudo_alg.tex <==
\section{Pseudo-likelihood algorithm}\label{sec:pseudo}

Instead of analyzing the weighted network through the weights of each edge, as it is considered in the likelihood function in \eqref{def:likelihood}, our goal is to summarize the node information through the sum of the edges weights connected to it. This methodology is approached in the case of unweighted networks in \cite{amini2013pseudo}.

Let $e=(e_1,\dots,e_n)\in \{1,\dots ,K\}^n$ be a labeling vector of the nodes. For $i=1,\dots,n$ and $k=1,\dots,K$, we define $s_{ik}(e)$ as the sum of the edges weights connected to node $i$ that belongs to community $k$, that is, 
\begin{equation}\label{def:block_sum}
s_{ik}(e) = \sum\limits_{j=1}^nW_{ij}\ind\{e_j=k\}\,.
\end{equation}

For each node $i$, define the vector of block sums $\mathbf{s}_i(e)=(s_{i1}(e),\dots,s_{iK}(e))$. Let $R$ be the $K\times K$ confusion matrix with $(k,l)$-th entry given by
\begin{equation}
R_{kl} = \dfrac{1}{n}\sum\limits_{i=1}^n\ind\{e_i=k,c_i=l\}\,.
\end{equation}

Conditioned on the true labels $c$, $\{s_{i1}(e),\dots,s_{iK}(e)\}$ are mutually independent random variables. 
Moreover, for each node $i$, conditioned on the labels $c=(c_1,\dots,c_n)$ with $c_i=l$, we have that
\begin{equation}\label{eq:gaussian_s}
s_{ik}(e)\sim N(P_{lk}\,,\Lambda_{lk})\,,
\end{equation}
with $P_{lk}=nR_{k}.B._{l}$ and $\Lambda_{lk}=nR_{k}.\Sigma._{l}$, where for a matrix $M$, $M_{k}.$ denotes the $k$th row of $M$ and $M._{k}$ denotes the $k$th column of $M$. In this way, the new matrices $P$ and $\Lambda$ are obtained by a mixture of the true parameters $B$ and $\Sigma$ using as mixture function the proportion of misclassified nodes of community assignment $e$ through the confusion matrix $R$.

%{\color{red} should we write the computation of the mean $P$ and variance $\Lambda$? should I add this computation in the appendix ?}

Each random vector $\mathbf{s}_i(e)$ can be written as a mixture of Gaussian random vectors with latent variables given by the true label $c_i$, that is, 
\begin{equation}
p(\,\mathbf{s_i}(e)\,|\,\pi,P,\Lambda) = \sum\limits_{l=1}^K\,\pi_l\,p(\,\mathbf{s_i}(e)\,|\,P_{l}.\,,\Lambda_{l}.)\,.
\end{equation}
%
%\begin{equation}
%p(\mathbf{s_i}\,|\,\pi,P,\Lambda) = \sum\limits_{l=1}^K\,\pi_l\,p(\mathbf{s_i}\,|\,P,\Lambda,c_i=l)
%\end{equation}

Due to the symmetry of $W$, %since $W$ is symmetric,% 
for each pair of nodes $i$ and $j$, $s_{ik}(e)$ and $s_{jk}(e)$ are not independent random variables. In our approach, the dependence between the variables $\{\mathbf{s}_1(e),\dots,\mathbf{s}_n(e)\}$ is ignored and the distribution $p(\,\mathbf{s_i}(e)\,|\,P_{l}.\,,\Lambda_{l}.)$ is written by the product of the Gaussian random variables in \eqref{eq:gaussian_s}. Thus, the pseudo log-likelihood (up to a constant) can be written as
\begin{equation}\label{def:pseudo}
\ell_{_{PL}}(\pi,P,\Lambda;\{\mathbf{s_i}(e)\}) = \sum\limits_{i=1}^n\log\left(  \sum\limits_{l=1}^K\,\pi_l \prod\limits_{k=1}^K\dfrac{1}{\sqrt{\Lambda_{lk}}}\exp\left\lbrace \dfrac{- (s_{ik}(e)-P_{lk})^2}{2\Lambda_{lk}} \right\rbrace \right)
\end{equation}

The pseudo-likelihood can be interpreted as a Gaussian mixture model where the mixture distribution corresponds to the distribution $\pi$ of the hidden communities labels $c=(c_1,\dots,c_n)$. We can obtain a pseudo-likelihood estimate of $(\pi,P,\Lambda)$ by maximizing the function \eqref{def:pseudo} using the EM algorithm with initial labeling $e$. Each step of the EM algorithm updates the parameters values using the community probability estimates until convergence. After that, the initial community labels $e$ is updated as the most likely label assignment using the current parameters estimates. This procedure is repeated for a fixed number of iterations $T$. At the end, the algorithm returns the most likely label assignment $\widehat{c}$ associated with the maximum pseudo-likelihood parameter estimates.

Given any community partition $e$, the estimators of $\pi$, $B$ and $\Sigma$ are obtained by maximizing the complete likelihood \eqref{def:joint}. In this way, we have that
\begin{equation}
\widehat{\pi}_k(e) = \frac{n_k(e)}{n}\,,
\end{equation}
\begin{equation}
\widehat{B}_{kl}(e) = \dfrac{1}{n_{kl}(e)}\sum\limits_{1\leq i < j \leq n}W_{ij}\mathds{1}\{e_i=k,e_j=l\}
\end{equation}
and
\begin{equation}
\widehat{\Sigma}_{kl}(e) = \dfrac{1}{n_{kl}(e)}\sum\limits_{1\leq i < j \leq n}(W_{ij}-\widehat{B}_{kl})^2\,\mathds{1}\{e_i=k,e_j=l\}\,.
\end{equation}

The EM algorithm applied to the mixture of Gaussian random variables is described in Algorithm \ref{alg:pseudo}. As it is usual, the performance of the EM algorithm depends on the choice of the initial labeling $e$. In our theoretical results, we show that it is only necessary to control the matching rate of the initial labeling $e$ and the true labels $c$. This scenario might be observed in real data when a fraction of nodes labels are known. However, in most of the cases, the information about the nodes membership is not available a priori. In this way, one possible manner to choose the initial labeling is to use the output of any other method as the initialization of the EM algorithm. The performance of the EM algorithm for different initialization labels is discussed in details in the simulation study carry out in Section \ref{sec:simulations}.    \\

\begin{algorithm}[H]
\caption{Pseudo-likelihood algorithm}
\label{alg:pseudo}
\begin{algorithmic}[1]
\State \textbf{Input:} Initial labeling $e$ and the weighted network $W$
\State \textbf{Output:} The labels estimates $\widehat{c}$\\
\State Compute $\widehat{\pi}_l(e)$, $\widehat{R}=diag(\widehat{\pi}_1,\dots,\widehat{\pi}_K)$, $\widehat{P}_{lk}=n\widehat{R}_{k}.\widehat{B}._{l}$ and $\widehat{\Lambda}_{lk}=n\widehat{R}_{k}.\widehat{\Sigma}._{l}$.
\State  \textbf{repeat} steps (6) - (11) $T$ times
\REPEAT 
\State Compute the block sums using \eqref{def:block_sum}.
\State Estimate the probabilities of node labels by
\begin{equation}
\widehat{\pi}_{il} = \mathbb{P}_{_{PL}}(c_i=l|\,\mathbf{s}_i(e)\,) = \dfrac{\,\widehat{\pi}_l \prod\limits_{k=1}^K\dfrac{1}{(\widehat{\Lambda}_{lk})^{1/2}}\exp\left\lbrace \dfrac{- (s_{ik}(e)-\widehat{P}_{lk})^2}{2\widehat{\Lambda}_{lk}} \right\rbrace}{\sum\limits_{m=1}^K\,\widehat{\pi}_m \prod\limits_{k=1}^K\dfrac{1}{(\widehat{\Lambda}_{mk})^{1/2}}\exp\left\lbrace \dfrac{- (s_{ik}(e)-\widehat{P}_{mk})^2}{2\widehat{\Lambda}_{mk}} \right\rbrace}\,.
\end{equation}
\State Update the parameter values
\begin{equation}
\widehat{\pi}_l=\dfrac{1}{n}\sum\limits_{i=1}^n\widehat{\pi}_{il}\,,\qquad \widehat{P}_{lk}=\dfrac{\sum\limits_{i=1}^n\widehat{\pi}_{il}s_{ik}(e)}{\sum\limits_{i=1}^n\widehat{\pi}_{il}}\quad\mbox{ and }\quad \widehat{\Lambda}_{lk}=\dfrac{\sum\limits_{i=1}^n\widehat{\pi}_{il}(s_{ik}(e)-\widehat{P}_{lk})^2}{\sum\limits_{i=1}^n\widehat{\pi}_{il}}\,.
\end{equation}
\UNTIL{the parameters estimates converge}
\State Update the labels by $e_i=\arg\max\limits_{l=1,\dots,K}\widehat{\pi}_{il}$ and return to (5).\\
\Return \textbf{Return:} $e$
\end{algorithmic}
\end{algorithm}

